Explicit Spatial Encoding for Deep Local Descriptors

We propose a kernelized deep local-patch descriptor based on efficient match kernels of neural network activations. Response of each receptive field is encoded together with its spatial location using explicit feature maps. Two location parametrizations, Cartesian and polar, are used to provide robustness to a different types of canonical patch misalignment. Additionally, we analyze how the conventional architecture, i.e. a fully connected layer attached after the convolutional part, encodes responses in a spatially variant way. In contrary, explicit spatial encoding is used in our descriptor, whose potential applications are not limited to local-patches. We evaluate the descriptor on standard benchmarks. Both versions, encoding 32x32 or 64x64 patches, consistently outperform all other methods on all benchmarks. The number of parameters of the model is independent of the input patch resolution.

==> app.tex <==
\begin{appendices}
\section{Explicit feature maps}
\label{sec:app}

As a non-linear kernel to compare scalars, \eg coordinates on the 2D grid, we use the normalized Von Mises (VM) probability density function~\cite{TBFJ15}, which is also known as the periodic normal distribution. It is parametrized by $\kappa$ controlling the shape of the kernel, where lower $\kappa$ corresponds to wider kernel. Following prior work~\cite{VZ10,TBFJ15,BTJ15}, we use the Fourier series approximation with $s$ frequencies that produces a feature map
\begin{equation}
\vspace{4pt}
\small
f(\alpha) = \left( \begin{array}{c} \sqrt{u_0} \\ \sqrt{u_1}\cos(\alpha) \\ \vdots \\ \sqrt{u_s}\cos(s\alpha) \\ \sqrt{u_1}\sin(\alpha) \\ \vdots \\ \sqrt{u_s}\sin(s\alpha) \end{array} \right),
\label{equ:featuremap}
\vspace{4pt}
\end{equation}
where $u_0, \ldots, u_s$ are the Fourier coefficients of the VM kernel $k_{VM}$.
It is easy to show that similarity of two such feature maps approximates the VM kernel with a Fourier series of $s+1$ terms
\begin{equation}
\vspace{4pt}
f(\alpha)^\top f(\beta) = \sum_{i=0}^s u_i \cos(i (\alpha-\beta)) \approx k_{VM}(\alpha-\beta).
\label{equ:vmapprox}
\vspace{4pt}
\end{equation}
Product $k(x_p\minust \alpha) \cdott k(y_p\minust \beta)$ in (\ref{equ:encsim}) \alert{can be seen as similar to a 2D RBF kernel} centered at $x_p, y_p$.
However, note that the final effect of the kernel depends on matrix $M$ as well, due to multiplication of the joint encoding~\cite{MTC17}. %
Such a feature map is applied to angles (scalars). We therefore map coordinates $x$, $y$, and $\rho$ uniformly to angles in $[0, \pi]$.

\end{appendices}


==> ext-plots.tex <==
\usepackage{tikzextern}
\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> no-plots.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\extdata}[1]{}


==> tables/hardnet_patchmaps.tex <==
\centering
\begin{tabular}{ccccc}
 \includegraphics[height=65pt]{patchmaps/hardnet/patch_0.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/patch_0.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/patch_1.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/patch_2.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/patch_3.png} \\
 \includegraphics[height=65pt]{patchmaps/hardnet/patch_0_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_0_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_1_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_2_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_3_pos_3_3.png} \\
 \includegraphics[height=65pt]{patchmaps/hardnet/patch_0_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_0_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_1_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_2_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_3_pos_1_3.png} \\
 \includegraphics[height=65pt]{patchmaps/hardnet/patch_0_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_0_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_1_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_2_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/hardnet/match_0_3_pos_4_4.png} \\
\end{tabular}



==> tables/hardnetnew_patchmaps.tex <==
\centering
\begin{tabular}{ccc}
 \includegraphics[height=65pt]{patchmaps/hardnetnew64/patch_0.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetnew64/patch_0.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetones/patch_0.png} \\
 \includegraphics[height=65pt]{patchmaps/hardnetnew64/patch_0_pos_6_6.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetnew64/match_0_0_pos_6_6.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetones/match_0_0_pos_3_3.png} \\
 \includegraphics[height=65pt]{patchmaps/hardnetnew64/patch_0_pos_2_6.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetnew64/match_0_0_pos_2_6.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetones/match_0_0_pos_1_3.png} \\
 \includegraphics[height=65pt]{patchmaps/hardnetnew64/patch_0_pos_8_8.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetnew64/match_0_0_pos_8_8.png}
  & \includegraphics[height=65pt]{patchmaps/hardnetones/match_0_0_pos_4_4.png} \\
\end{tabular}



==> tables/indep_patchmaps.tex <==
\centering
\begin{tabular}{ccccc}
 \includegraphics[height=65pt]{patchmaps/indep/patch_0.png}
  & \includegraphics[height=65pt]{patchmaps/indep/patch_0.png}
  & \includegraphics[height=65pt]{patchmaps/indep/patch_1.png}
  & \includegraphics[height=65pt]{patchmaps/indep/patch_2.png}
  & \includegraphics[height=65pt]{patchmaps/indep/patch_3.png} \\
 \includegraphics[height=65pt]{patchmaps/indep/patch_0_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_0_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_1_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_2_pos_3_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_3_pos_3_3.png} \\
 \includegraphics[height=65pt]{patchmaps/indep/patch_0_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_0_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_1_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_2_pos_1_3.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_3_pos_1_3.png} \\
 \includegraphics[height=65pt]{patchmaps/indep/patch_0_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_0_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_1_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_2_pos_4_4.png}
  & \includegraphics[height=65pt]{patchmaps/indep/match_0_3_pos_4_4.png} \\
\end{tabular}



==> tables/internal/match.tex <==
\begin{tikzpicture}
\begin{axis}[
width=\figW,
height=\figH,
at={(0\figW,0\figH)},
scale only axis,
clip=false,
xmin=35,
xmax=55,
xlabel={Image Matching mAP [\%]},
y dir=reverse,
ymin=0.6,
ymax=12.4,
ytick={1,2,3,4,5,6,7,8,9,10,11,12},
yticklabels={{\tiny \dessum},{\tiny  \descat},{\tiny  \carta},{\tiny  \polara},{\tiny  \cartb},{\tiny  \polarb},{\tiny  \indepa},{\tiny  \hardnet},{\tiny  \noindep},{\tiny  \indepb},{\tiny  \indepb(64)},{\tiny \hardnet(64)}},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]

\addplot[xbar, bar width=0.8, fill=colnsum, draw=black, area legend] table[row sep=crcr] {%
38.18 1\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,1) { 38.18 {\tiny \pmm 0.17 } };

\addplot[xbar, bar width=0.8, fill=colncat, draw=black, area legend] table[row sep=crcr] {%
51.30 2\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,2) { 51.30  };

\addplot[xbar, bar width=0.8, fill=colcrta, draw=black, area legend] table[row sep=crcr] {%
51.83 4\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,4) { 51.83 {\tiny \pmm 0.04 } };

\addplot[xbar, bar width=0.8, fill=colpola, draw=black, area legend] table[row sep=crcr] {%
51.94 3\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,3) { 51.94 {\tiny \pmm 0.09 } };

\addplot[xbar, bar width=0.8, fill=colcrtb, draw=black, area legend] table[row sep=crcr] {%
52.58 6\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,6) { 52.58 {\tiny \pmm 0.06 } };

\addplot[xbar, bar width=0.8, fill=colpolb, draw=black, area legend] table[row sep=crcr] {%
52.96 5\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,5) { 52.96 {\tiny \pmm 0.05 } };

\addplot[xbar, bar width=0.8, fill=colinda, draw=black, area legend] table[row sep=crcr] {%
52.96 7\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,7) { 52.96 {\tiny \pmm 0.16 } };

\addplot[xbar, bar width=0.8, fill=colhard, draw=black, area legend] table[row sep=crcr] {%
53.09 8\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,8) { 53.09 {\tiny \pmm 0.15 } };

\addplot[xbar, bar width=0.8, fill=colnind, draw=black, area legend] table[row sep=crcr] {%
53.06 9\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,9) { 53.06 {\tiny \pmm 0.07 } };

\addplot[xbar, bar width=0.8, fill=colindb, draw=black, area legend] table[row sep=crcr] {%
53.73 10\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,10) { 53.73 {\tiny \pmm 0.07 } };

\addplot[xbar, bar width=0.8, fill=colindb64, draw=black, area legend] table[row sep=crcr] {%
54.24 11\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,11) { 54.24 {\tiny \pmm 0.07 } };

\addplot[xbar, bar width=0.8, fill=colhard64, draw=black, area legend] table[row sep=crcr] {%
53.50 12\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
35  0.6\\
35  12.4\\
};
\node[right, align=left]
at (axis cs:55.2,12) { 53.50 {\tiny \pmm 0.12 } };
\end{axis}
\end{tikzpicture}


==> tables/internal/retrv.tex <==
\begin{tikzpicture}
\begin{axis}[
width=\figW,
height=\figH,
at={(0\figW,0\figH)},
scale only axis,
clip=false,
xmin=60,
xmax=75,
xlabel={Image Retrieval mAP [\%]},
y dir=reverse,
ymin=0.6,
ymax=12.4,
ytick={1,2,3,4,5,6,7,8,9,10,11,12},
yticklabels={{\tiny \dessum},{\tiny  \descat},{\tiny  \carta},{\tiny  \polara},{\tiny  \cartb},{\tiny  \polarb},{\tiny  \indepa},{\tiny  \hardnet},{\tiny  \noindep},{\tiny  \indepb},{\tiny  \indepb(64)},{\tiny \hardnet(64)}},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]

\addplot[xbar, bar width=0.8, fill=colnsum, draw=black, area legend] table[row sep=crcr] {%
61.97 1\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,1) { 61.97 {\tiny \pmm 0.18 } };

\addplot[xbar, bar width=0.8, fill=colncat, draw=black, area legend] table[row sep=crcr] {%
69.91 2\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,2) { 69.91  };

\addplot[xbar, bar width=0.8, fill=colcrta, draw=black, area legend] table[row sep=crcr] {%
71.39 4\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,4) { 71.39 {\tiny \pmm 0.01 } };

\addplot[xbar, bar width=0.8, fill=colpola, draw=black, area legend] table[row sep=crcr] {%
71.22 3\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,3) { 71.22 {\tiny \pmm 0.08 } };

\addplot[xbar, bar width=0.8, fill=colcrtb, draw=black, area legend] table[row sep=crcr] {%
71.61 6\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,6) { 71.61 {\tiny \pmm 0.09 } };

\addplot[xbar, bar width=0.8, fill=colpolb, draw=black, area legend] table[row sep=crcr] {%
71.51 5\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,5) { 71.51 {\tiny \pmm 0.05 } };

\addplot[xbar, bar width=0.8, fill=colinda, draw=black, area legend] table[row sep=crcr] {%
72.14 7\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,7) { 72.14 {\tiny \pmm 0.1 } };

\addplot[xbar, bar width=0.8, fill=colhard, draw=black, area legend] table[row sep=crcr] {%
71.26 8\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,8) { 71.26 {\tiny \pmm 0.1 } };

\addplot[xbar, bar width=0.8, fill=colnind, draw=black, area legend] table[row sep=crcr] {%
71.72 9\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,9) { 71.72 {\tiny \pmm 0.08 } };

\addplot[xbar, bar width=0.8, fill=colindb, draw=black, area legend] table[row sep=crcr] {%
72.29 10\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,10) { 72.29 {\tiny \pmm 0.08 } };

\addplot[xbar, bar width=0.8, fill=colindb64, draw=black, area legend] table[row sep=crcr] {%
72.54 11\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,11) { 72.54 {\tiny \pmm 0.02 } };

\addplot[xbar, bar width=0.8, fill=colhard64, draw=black, area legend] table[row sep=crcr] {%
71.49 12\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
60  0.6\\
60  12.4\\
};
\node[right, align=left]
at (axis cs:75.2,12) { 71.49 {\tiny \pmm 0.12 } };
\end{axis}
\end{tikzpicture}


==> tables/internal/verif.tex <==
\begin{tikzpicture}
\begin{axis}[
width=\figW,
height=\figH,
at={(0\figW,0\figH)},
scale only axis,
clip=false,
xmin=80,
xmax=90,
xlabel={Image Verification mAP [\%]},
y dir=reverse,
ymin=0.6,
ymax=12.4,
ytick={1,2,3,4,5,6,7,8,9,10,11,12},
yticklabels={{\tiny \dessum},{\tiny  \descat},{\tiny  \carta},{\tiny  \polara},{\tiny  \cartb},{\tiny  \polarb},{\tiny  \indepa},{\tiny  \hardnet},{\tiny  \noindep},{\tiny  \indepb},{\tiny  \indepb(64)},{\tiny \hardnet(64)}},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]

\addplot[xbar, bar width=0.8, fill=colnsum, draw=black, area legend] table[row sep=crcr] {%
84.29 1\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,1) { 84.29 {\tiny \pmm 0.11 } };

\addplot[xbar, bar width=0.8, fill=colncat, draw=black, area legend] table[row sep=crcr] {%
86.92 2\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,2) { 86.92  };

\addplot[xbar, bar width=0.8, fill=colcrta, draw=black, area legend] table[row sep=crcr] {%
88.37 4\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,4) { 88.37 {\tiny \pmm 0.04 } };

\addplot[xbar, bar width=0.8, fill=colpola, draw=black, area legend] table[row sep=crcr] {%
88.70 3\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,3) { 88.70 {\tiny \pmm 0.02 } };

\addplot[xbar, bar width=0.8, fill=colcrtb, draw=black, area legend] table[row sep=crcr] {%
88.64 6\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,6) { 88.64 {\tiny \pmm 0.09 } };

\addplot[xbar, bar width=0.8, fill=colpolb, draw=black, area legend] table[row sep=crcr] {%
88.72 5\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,5) { 88.72 {\tiny \pmm 0.04 } };

\addplot[xbar, bar width=0.8, fill=colinda, draw=black, area legend] table[row sep=crcr] {%
89.02 7\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,7) { 89.02 {\tiny \pmm 0.13 } };

\addplot[xbar, bar width=0.8, fill=colhard, draw=black, area legend] table[row sep=crcr] {%
88.61 8\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,8) { 88.61 {\tiny \pmm 0.04 } };

\addplot[xbar, bar width=0.8, fill=colnind, draw=black, area legend] table[row sep=crcr] {%
88.87 9\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,9) { 88.87 {\tiny \pmm 0.07 } };

\addplot[xbar, bar width=0.8, fill=colindb, draw=black, area legend] table[row sep=crcr] {%
89.16 10\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,10) { 89.16 {\tiny \pmm 0.06 } };

\addplot[xbar, bar width=0.8, fill=colindb64, draw=black, area legend] table[row sep=crcr] {%
89.45 11\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,11) { 89.45 {\tiny \pmm 0.04 } };

\addplot[xbar, bar width=0.8, fill=colhard64, draw=black, area legend] table[row sep=crcr] {%
88.68 12\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
80  0.6\\
80  12.4\\
};
\node[right, align=left]
at (axis cs:90.2,12) { 88.68 {\tiny \pmm 0.08 } };
\end{axis}
\end{tikzpicture}


==> tables/stateofart/match.tex <==
\begin{tikzpicture}
\begin{axis}[
 width=\figW,
 height=\figH,
 at={(0\figW,0\figH)},
 scale only axis,
 clip=false,
 xmin=0,
 xmax=60,
 xlabel={Image Matching mAP [\%]},
 y dir=reverse,
 ymin=0.6,
 ymax=16.4,
 ytick={1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15, 16},
 yticklabels={\brief, \binboost, \orb, \dcsiam, \sift, \rootsift, \dcsiamts, \deepdesc, \tfmargin, \mkd, \lnet, \hardnet$\dagger$, \hardnet, \hardnet(64), \indepb, \indepb(64)},
 axis background/.style={fill=white},
 xmajorgrids,
 ymajorgrids
 ]

\addplot[xbar, bar width=0.8, fill=mycolor12, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
10.288200  1\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,1) {10.29};

\addplot[xbar, bar width=0.8, fill=mycolor5, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
14.722800  2\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,2) {14.72};

\addplot[xbar, bar width=0.8, fill=mycolor3, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
15.164300  3\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,3) {15.16};

\addplot[xbar, bar width=0.8, fill=mycolor9, draw=black, area legend] table[row sep=crcr] {%
25.098800  4\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,4) {25.10};

\addplot[xbar, bar width=0.8, fill=mycolor6, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
25.780300  5\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,5) {25.78};

\addplot[xbar, bar width=0.8, fill=mycolor7, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
27.212400  6\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,6) {27.21};

\addplot[xbar, bar width=0.8, fill=mycolor10, draw=black, area legend] table[row sep=crcr] {%
27.763900  7\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,7) {27.76};

\addplot[xbar, bar width=0.8, fill=mycolor8, draw=black, area legend] table[row sep=crcr] {%
28.340800  8\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,8) {28.34};

\addplot[xbar, bar width=0.8, fill=mycolor11, draw=black, area legend] table[row sep=crcr] {%
32.761500  9\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,9) {32.76};

\addplot[xbar, bar width=0.8, fill=mycolor4, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
37.160000  10\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,10) {37.16};

\addplot[xbar, bar width=0.8, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
45.491100  11\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,11) {45.49};

\addplot[xbar, bar width=0.8, fill=colhardr, draw=black, area legend] table[row sep=crcr] {%
52.76  12\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,12) {52.76};

\addplot[xbar, bar width=0.8, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
53.09  13\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,13) {53.09};

\addplot[xbar, bar width=0.8, fill=colhard64, draw=black, area legend] table[row sep=crcr] {%
53.5  14\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0  0.6\\
0  16.4\\
};
\node[right, align=left]
at (axis cs:61,14) {53.50};

\addplot[xbar, bar width=0.8, fill=colindb, draw=black, area legend] table[row sep=crcr] {%
53.73 15\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,15) {53.73};

\addplot[xbar, bar width=0.8, fill=colindb64, draw=black, area legend] table[row sep=crcr] {%
54.24  16\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:61,16) {54.24};

\end{axis}
\end{tikzpicture}


==> tables/stateofart/retrv.tex <==
\begin{tikzpicture}
\begin{axis}[
 width=\figW,
 height=\figH,
 at={(0\figW,0\figH)},
 scale only axis,
 clip=false,
 xmin=0,
 xmax=80,
 xlabel={Patch Retrieval mAP [\%]},
 y dir=reverse,
 ymin=0.6,
 ymax=16.4,
 ytick={1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15, 16},
 yticklabels={\brief, \orb, \binboost, \sift, \rootsift, \dcsiamts, \dcsiam, \tfmargin, \mkd, \deepdesc, \lnet, \hardnet$\dagger$, \hardnet, \hardnet(64), \indepb, \indepb(64)},
 axis background/.style={fill=white},
 xmajorgrids,
 ymajorgrids
 ]

\addplot[xbar, bar width=0.8, fill=mycolor12, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
26.317700  1\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,1) {26.32};

\addplot[xbar, bar width=0.8, fill=mycolor3, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
29.518600  2\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,2) {29.52};

\addplot[xbar, bar width=0.8, fill=mycolor5, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
34.180100  3\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,3) {34.18};

\addplot[xbar, bar width=0.8, fill=mycolor6, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
43.040300  4\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,4) {43.04};

\addplot[xbar, bar width=0.8, fill=mycolor7, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
43.264200  5\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,5) {43.26};

\addplot[xbar, bar width=0.8, fill=mycolor10, draw=black, area legend] table[row sep=crcr] {%
47.566500  6\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,6) {47.57};

\addplot[xbar, bar width=0.8, fill=mycolor9, draw=black, area legend] table[row sep=crcr] {%
48.528400  7\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,7) {48.53};

\addplot[xbar, bar width=0.8, fill=mycolor11, draw=black, area legend] table[row sep=crcr] {%
52.413000  8\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,8) {52.41};

\addplot[xbar, bar width=0.8, fill=mycolor4, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
53.500000  9\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,9) {53.50};

\addplot[xbar, bar width=0.8, fill=mycolor8, draw=black, area legend] table[row sep=crcr] {%
53.981000  10\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,10) {53.98};

\addplot[xbar, bar width=0.8, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
63.587500  11\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,11) {63.59};

\addplot[xbar, bar width=0.8, fill=colhardr, draw=black, area legend] table[row sep=crcr] {%
69.66  12\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,12) {69.66};

\addplot[xbar, bar width=0.8, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
71.26  13\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,13) {71.26};

\addplot[xbar, bar width=0.8, fill=colhard64, draw=black, area legend] table[row sep=crcr] {%
71.49  14\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0  0.6\\
0  16.4\\
};
\node[right, align=left]
at (axis cs:81,14) {71.49};

\addplot[xbar, bar width=0.8, fill=colindb, draw=black, area legend] table[row sep=crcr] {%
72.29  15\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,15) {72.29};

\addplot[xbar, bar width=0.8, fill=colindb64, draw=black, area legend] table[row sep=crcr] {%
72.54  16\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:81,16) {72.54};


\end{axis}
\end{tikzpicture}


==> tables/stateofart/verif.tex <==
\begin{tikzpicture}
\begin{axis}[
 width=\figW,
 height=\figH,
 at={(0\figW,0\figH)},
 scale only axis,
 clip=false,
 xmin=0,
 xmax=100,
 xlabel={Patch Verification mAP [\%]},
 y dir=reverse,
 ymin=0.6,
 ymax=16.4,
 ytick={1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15, 16},
 yticklabels={\rootsift, \brief, \orb, \sift, \binboost, \dcsiam, \dcsiamts, \mkd, \deepdesc, \tfmargin, \lnet, \hardnet$\dagger$, \hardnet, \hardnet(64), \indepb, \indepb(64)},
 axis background/.style={fill=white},
 xmajorgrids,
 ymajorgrids
 ]

\addplot[xbar, bar width=0.8, fill=mycolor7, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
57.211 1\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,1) {57.21};

\addplot[xbar, bar width=0.8, fill=mycolor12, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
57.899  2\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,2) {57.90};

\addplot[xbar, bar width=0.8, fill=mycolor3, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
59.744  3\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,3) {59.74};

\addplot[xbar, bar width=0.8, fill=mycolor6, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
64.386  4\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,4) {64.39};

\addplot[xbar, bar width=0.8, fill=mycolor5, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
66.462  5\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,5) {66.46};

\addplot[xbar, bar width=0.8, fill=mycolor9, draw=black, area legend] table[row sep=crcr] {%
70.027  6\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,6) {70.03};

\addplot[xbar, bar width=0.8, fill=mycolor10, draw=black, area legend] table[row sep=crcr] {%
77.900  7\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,7) {77.90};

\addplot[xbar, bar width=0.8, fill=mycolor4, draw=black, postaction={pattern=north east lines}, area legend] table[row sep=crcr] {%
78.81  8\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,8) {78.81};

\addplot[xbar, bar width=0.8, fill=mycolor8, draw=black, area legend] table[row sep=crcr] {%
79.178  9\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,9) {79.18};

\addplot[xbar, bar width=0.8, fill=mycolor11, draw=black, area legend] table[row sep=crcr] {%
81.358  10\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,10) {81.36};

\addplot[xbar, bar width=0.8, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
86.381  11\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,11) {86.38};

\addplot[xbar, bar width=0.8, fill=colhardr, draw=black, area legend] table[row sep=crcr] {%
88.43  12\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,12) {88.43};

\addplot[xbar, bar width=0.8, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
88.61  13\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,13) {88.61};

\addplot[xbar, bar width=0.8, fill=colhard64, draw=black, area legend] table[row sep=crcr] {%
88.68  14\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0  0.6\\
0  16.4\\
};
\node[right, align=left]
at (axis cs:101,14) {88.68};

\addplot[xbar, bar width=0.8, fill=colindb, draw=black, area legend] table[row sep=crcr] {%
89.16  15\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,15) {89.16};

\addplot[xbar, bar width=0.8, fill=colindb64, draw=black, area legend] table[row sep=crcr] {%
89.45  16\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0	0.6\\
0	16.4\\
};
\node[right, align=left]
at (axis cs:101,16) {89.45};

\end{axis}
\end{tikzpicture}

